True Online Emphatic TD($\lambda$): Quick Reference and Implementation Guide

This document is a guide to the implementation of true online emphatic TD($\lambda$), a model-free temporal-difference algorithm for learning to make long-term predictions which combines the emphasis idea (Sutton, Mahmood & White 2015) and the true-online idea (van Seijen & Sutton 2014). The setting used here includes linear function approximation, the possibility of off-policy training, and all the generality of general value functions, as well as the emphasis algorithm's notion of "interest".

==> symbols.tex <==
\newdimen\pHeight
\pHeight=-32678sp
\newdimen\pLower
\pLower=-4096sp
\newdimen\pLineWidth
\pLineWidth=32678sp
\newdimen\pKern
\pKern=-276480sp
\newdimen\pIR
\pIR=-131072sp
\newsavebox{\Cbox}
\newsavebox{\vertCmplx}
\newdimen\Cheight
\newdimen\Cwidth
\sbox{\Cbox}{\rm C}
\Cheight=\ht\Cbox
\Cwidth=\wd\Cbox
\advance\Cheight by \pHeight
\sbox{\vertCmplx}{\rule[\pLower]{\pLineWidth}{\Cheight}}
\sbox{\Cbox}{\usebox{\Cbox}\kern\pKern\usebox{\vertCmplx}}
\wd\Cbox=\Cwidth
%\def\C{\usebox{\Cbox}}
%\def\Re{{\rm I\kern\pIR R}}
\def\Re{\mathbb{R}}
\def\Repart{\mathrm{Re}}
\def\Nat{{\rm I\kern\pIR N}}
\def\argmax{\mathop{\rm arg\,max}}
\def\argmin{\mathop{\rm arg\,min}}
\def\liminf{\mathop{\rm lim\,inf}}
\def\log{\mathop{\rm log}}
\def\Mean{{\bf Mean}}
\def\Var{{\bf Var}}
\def\Cov{{\bf Cov}}
\def\exptE{{\bf E}}
\newcommand{\EE}[2]{\mathbb{E}_{#1\!\!}\left[#2\right]}
\newcommand{\EEpi}[1]{\EE{\pi}{#1}}
\def\diag{\mathop{\rm diag}}

\def\setC{\mathbb{C}}

\def\A{{\mathcal{A}}}
\def\C{{\mathcal{C}}}
\def\D{{\mathcal{D}}}
\def\E{{\mathcal{E}}}
\def\F{{\mathcal{F}}}
\def\G{{\mathcal{G}}}
\def\H{{\mathcal{H}}}
\def\I{{\mathcal{I}}}
\def\J{{\mathcal{J}}}
\def\L{{\mathcal{L}}}
\def\M{{\mathcal{M}}}
\def\N{{\mathcal{N}}}
\def\O{{\mathcal{O}}}
\def\P{{\mathcal{P}}}
\def\Q{{\mathcal{Q}}}
\def\R{{\mathcal{R}}}
\def\S{{\mathcal{S}}}
\def\T{{\mathcal{T}}}
\def\U{{\mathcal{U}}}
\def\V{{\mathcal{V}}}
\def\W{{\mathcal{W}}}
\def\X{{\mathcal{X}}}
\def\Z{{\mathcal{Z}}}

\def\vecalpha{{\boldsymbol{\alpha}}}
\def\vectheta{{\boldsymbol{\theta}}}
\def\vecpi{{\boldsymbol{\pi}}}
\def\vecpsi{{\boldsymbol{\psi}}}
\def\vecphi{{\boldsymbol{\phi}}}
\def\vecmu{{\boldsymbol{\mu}}}
\def\vecdelta{{\boldsymbol{\delta}}}
%\def\vec0{{\boldsymbol{0}}}
\def\vecb{{\boldsymbol{b}}}
\def\vece{{\boldsymbol{e}}}
\def\vecf{{\boldsymbol{f}}}
\def\veck{{\boldsymbol{k}}}
\def\vecp{{\boldsymbol{p}}}
\def\vecq{{\boldsymbol{q}}}
\def\vecr{{\boldsymbol{r}}}
\def\vecu{{\boldsymbol{u}}}
\def\vecv{{\boldsymbol{v}}}
\def\vecw{{\boldsymbol{w}}}
\def\vecx{{\boldsymbol{x}}}
\def\vecy{{\boldsymbol{y}}}
\def\vecz{{\boldsymbol{z}}}

\def\matSigma{{\boldsymbol{\Sigma}}}
\def\matLambda{{\boldsymbol{\Lambda}}}
\def\matA{{\boldsymbol{A}}}
\def\hmatA{{\boldsymbol{\hat{A}}}}
\def\matC{{\boldsymbol{C}}}
\def\matD{{\boldsymbol{D}}}
\def\matF{{\boldsymbol{F}}}
\def\matG{{\boldsymbol{G}}}
\def\matH{{\boldsymbol{H}}}
\def\matI{{\boldsymbol{I}}}
\def\matK{{\boldsymbol{K}}}
\def\matP{{\boldsymbol{P}}}
\def\matU{{\boldsymbol{U}}}
\def\matX{{\boldsymbol{X}}}
\def\matY{{\boldsymbol{Y}}}
\def\matZ{{\boldsymbol{Z}}}

\newcommand{\ovs}{\overline{s}}
\newcommand{\ovr}{\overline{r}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{defn}[thm]{Definition}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary} %[thm]
\newtheorem{fact}[thm]{Fact}

\newcommand{\lambdamin}{\lambda_{\min}}
\newcommand{\lambdamax}{\lambda_{\max}}
\newcommand{\sigmamin}{\sigma_{\min}}
\newcommand{\sigmamax}{\sigma_{\max}}
\newcommand{\ra}{\rightarrow}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}
\def\real{\mathbb{R}}
\newcommand{\RealPart}{\mathrm{Re}}
\newcommand{\half}{{\frac12}} 
\newcommand\norm[1]{\|#1\|_2}
